Folding Branched Covers of the $3$-Sphere Branched over Knots

A folding of a branched cover of the 3-sphere that is branched over a knot is a continuous map of the cover into the product of the sphere with a disk that has the property that the projection onto the sphere factor induces the covering. Moreover, away from the branch set, the map is a general position immersion. Cyclic branched covers can be folded so that the map is an embedding when the disk factor is 2-dimensional. Dihedral branched covers can also be folded. In as much as possible, the foldings that are presented are quite detailed. In particular, the paper focuses upon a folding of the dihedral cover of the 3-sphere that is branched along a torus knot of type (2,5). The cover also is homeomorphic to the $3$-sphere.

==> reference.tex <==
@article {KamJKTR,
    AUTHOR = {Kamada, Seiichi},
     TITLE = {Surfaces in {${\bf R}^4$} of braid index three are ribbon},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {1},
      YEAR = {1992},
    NUMBER = {2},
     PAGES = {137--160},
      ISSN = {0218-2165,1793-6527},
   MRCLASS = {57Q45 (57M15 57M25)},
  MRNUMBER = {1164113},
MRREVIEWER = {Don\v co\ Dimovski},
       DOI = {10.1142/S0218216592000082},
       URL = {https://doi.org/10.1142/S0218216592000082},
}


@article {NS1,
    AUTHOR = {Nagase, Teruo and Shima, Akiko},
     TITLE = {On surface braids of index four with at most two crossings},
   JOURNAL = {Fund. Math.},
  FJOURNAL = {Fundamenta Mathematicae},
    VOLUME = {188},
      YEAR = {2005},
     PAGES = {167--193},
      ISSN = {0016-2736,1730-6329},
   MRCLASS = {57Q45 (57Q35)},
  MRNUMBER = {2191945},
MRREVIEWER = {Seiichi\ Kamada},
       DOI = {10.4064/fm188-0-9},
       URL = {https://doi.org/10.4064/fm188-0-9},
}


@article {NS2,
    AUTHOR = {Nagase, Teruo and Shima, Akiko},
     TITLE = {The structure of a minimal {$n$}-chart with two crossings {I}:
              {C}omplementary domains of {$\Gamma_1\cup\Gamma_{n-1}$}},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {27},
      YEAR = {2018},
    NUMBER = {14},
     PAGES = {1850078, 37},
      ISSN = {0218-2165,1793-6527},
   MRCLASS = {57Q45 (57Q35)},
  MRNUMBER = {3896318},
MRREVIEWER = {Arkadiy\ Skopenkov},
       DOI = {10.1142/S0218216518500785},
       URL = {https://doi.org/10.1142/S0218216518500785},
}


@book {KamBook,
     AUTHOR = {Kamada, Seiichi},
      TITLE = {Braid and knot theory in dimension four},
     SERIES = {Mathematical Surveys and Monographs},
  PUBLISHER = {American Mathematical Society},
       YEAR = {2002},
      PAGES = {xiv+313 pp.},
       ISBN = {0-8218-2969-6},
    MRCLASS = {57Q45 (20F36\\57M25\\57Q35)}},
   MRNUMBER = {1900979},
 MRREVIEWER = {Saito, Masahico},
        DOI = {10.1090/surv/095},
        URL = {https://doi.org/10.1090/surv/095},
}


@incollection {CSFold,
    AUTHOR = {Carter, J. Scott and Kamada, Seiichi},
     TITLE = {How to fold a manifold},
 BOOKTITLE = {New ideas in low dimensional topology},
    SERIES = {Ser. Knots Everything},
    VOLUME = {56},
     PAGES = {31--77},
 PUBLISHER = {World Sci. Publ., Hackensack, NJ},
      YEAR = {2015},
      ISBN = {978-981-4630-61-0},
   MRCLASS = {57M12 (57M25)},
  MRNUMBER = {3381322},
MRREVIEWER = {Luisa\ Paoluzzi},
       DOI = {10.1142/9789814630627\_0002},
       URL = {https://doi.org/10.1142/9789814630627_0002},
}


@book {Rolfsen,
    AUTHOR = {Rolfsen, Dale},
     TITLE = {Knots and links},
    SERIES = {Mathematics Lecture Series},
    VOLUME = {No. 7},
 PUBLISHER = {Publish or Perish, Inc., Berkeley, CA},
      YEAR = {1976},
     PAGES = {ix+439},
   MRCLASS = {55-01},
  MRNUMBER = {515288},
}


@incollection {KirSch,
    AUTHOR = {Kirby, R. C. and Scharlemann, M. G.},
     TITLE = {Eight faces of the {P}oincar\'{e} homology {$3$}-sphere},
 BOOKTITLE = {Geometric topology ({P}roc. {G}eorgia {T}opology {C}onf.,
              {A}thens, {G}a., 1977)},
     PAGES = {113--146},
 PUBLISHER = {Academic Press, New York-London},
      YEAR = {1979},
      ISBN = {0-12-158860-2},
   MRCLASS = {57Q45 (14B05 32B30)},
  MRNUMBER = {537730},
MRREVIEWER = {Anatoly\ Libgober},
}


@incollection {QuickTrip,
    AUTHOR = {Fox, R. H.},
     TITLE = {A quick trip through knot theory},
 BOOKTITLE = {Topology of 3-manifolds and related topics ({P}roc. {T}he
              {U}niv. of {G}eorgia {I}nstitute, 1961)},
     PAGES = {120--167},
 PUBLISHER = {Prentice-Hall, Inc., Englewood Cliffs, NJ},
      YEAR = {1961},
   MRCLASS = {55.20},
  MRNUMBER = {140099},
MRREVIEWER = {L.\ Neuwirth},
}


